Quantum Walks

This tutorial article showcases the many varieties and uses of quantum walks. Discrete time quantum walks are introduced as counterparts of classical random walks. The emphasis is on the connections and differences between the two types of processes (with rather different underlying dynamics) for producing random distributions. We discuss algorithmic applications for graph-searching and compare the two approaches. Next, we look at quantization of Markov chains and show how it can lead to speedups for sampling schemes. Finally, we turn to continuous time quantum walks and their applications, which provide interesting (even exponential) speedups over classical approaches.

==> chap0intro.tex <==
%!TEX root = APSwalks.tex
%=============================================================================================
\section{Classical Random Walks}

To amuse students, or to catch their attention, it is quite usual to start statistical mechanics university courses with the \emph{drunkard's walk} example. We are told the story of a drunken sailor who gets so drunk that the probability for him to move forward on his way home is equal to the probability to move backward to the tavern where he likes to spend most of his time when he is not at sea. Looking at him at some point between the tavern and his home and letting him make a number of drunken steps, we ask where will we find him with the highest probability?

This seemingly trivial problem is very important. In fact, it can be retold in many various ways. For example the \emph{Galton's board} \cite{Galton89} device, also known as the \emph{quincunx} (see Fig.~\ref{fig-17}b), has the same properties as the drunkard's walk. Balls are dropped from the top orifice and as they move downward, they bounce and scatter off the pins. Finally, they gather and rest in the boxes on the bottom. The number of balls in a box some distance from the horizontal position of the orifice can be mapped (is proportional) to the probability for the drunken sailor to be found at a particular distance from the tavern (after a specific number of steps corresponding to the vertical dimension of the quincunx). This is due to the fact, that the ball on its way downward scatters from the pins with approximately the same probability to the left as to the right --- it moves in the same manner as the sailor on his way from the tavern. Another retelling of the sailor's story is the magnetization of an ideal paramagnetic gas\footnote{It is an ensamble of magnetic particles (in this case without any external field), that do not interact --- they do not feel each other.} of spin-$1/2$ particles. Tossing a coin is yet another example of drunkard's walk.

\begin{figure}
\begin{center}
\includegraphics{chap1_quincunx.pdf}
\end{center}
\caption{A possible realization of the drunkard's walk -- the quincunx (Galton's board). The number of marbles in a bin at the bottom correspond to the probability of the sailor to be at that position after taking 19 random steps (the number of pins a falling marble encounters on its way down).}\label{fig-17}
\end{figure}

This simple {\em walk on a line} is not just an example of some simple problems. It serves as a toy model and starting point for more involved variations. These modifications of the drunkard's walk spread across many branches of science and their position is justified by the results they provide. The roots of random walks, however, lie in the areas of mathematics, economy and physics. Probably the earliest (1900) attempt to describe random walks originates in the doctoral thesis of Bachelier \cite{Bachelier00}, who considered the evolution of market prices as a succession of random changes. His thesis, however, was not very rigorous and random walks had to wait to be defined properly from a mathematical viewpoint. This was done by Wiener \cite{Wiener23} in 1923. In physics it was Einstein \cite{Einstein05}, who in his theoretical paper on Brownian motion from 1905 put the first theoretical description of a random walk in natural sciences with explanation based on the kinetic theory, where gases (and liquids) are considered to be composed of many small colliding particles --- it was aimed to explain thermodynamical phenomena as statistical consequences of such movement of particles. Einstein speculated, that if (as he believed) the kinetic theory was right, then the seemingly random Brownian motion \cite{Brown} of large particles would be the result of the action of myriads of small solvent particles. Based on kinetic theory, he was able to describe the properties of the motion of the solute particles --- i.e.~connect the osmotic pressure of these particles with their density --- and show the connection with the diffusive process. Assuming the densities of solvent and solution are known, an experiment based on the barometric formula stating how the pressure changes with altitude provides us with the kinetic energy of solute particles at a given temperature. Hence, the Avogadro number can be estimated. This, indeed, has been done \cite{Perrin09} and strengthened the position of the kinetic theory at that time.

%=============================================================================================
\subsection{Markov Chains}
\label{sec:markov_chains}

Random walks have been formulated in many different ways. Generally, we say that a {\em random walk} is a succession of moves, generated in a stochastic (random) manner, inside a given state space $\Omega$ that generally has a more complex structure than a previously mentioned liear chain (drunkard's walk). If the stochastic moves are correlated in time, we talk about non-Markovian walks (walks with memory), however, for our purposes we will always assume the walks to be Markovian -- the random moves of the walker are uncorrelated in time. Note, though, that the stochastic generator may be position dependent.
The sequences of such moves result in the so-called \emph{Markov Chains}. 

Taking only one instance (path) of a random walk is, naturally, not enough to devise the general properties of the phenomenon of random walks. That is why we consider the evolution of distributions on state space $\Omega$. These distributions are the averages over many instances of a random walk of a single walker (or an ensemble of walkers). In such case, for a Markovian walk in a countable space\footnote{The topic of uncountable spaces is not important for the scope of this work.} $\Omega$, we define a distribution
\[
	p=\begin{pmatrix}
	p_1\\
	p_2\\
	p_3\\
	\vdots\end{pmatrix}
\]
over indexed states, with $p_k$ corresponding to the probability of finding the walker at the position with index $k$. For $p$ to define a probability, it is necessary that
\[
\sum_{k}p_k=1.
\]
In this framework, the stochastic generator that describes the single-step evolution of a distribution function is given as a stochastic matrix\footnote{A \emph{stochastic matrix} is a real matrix with columns summing to 1, which preserves the probability measure, i.e.~all its elements are positive and smaller than one.} $M$, giving the one-step evolution of a distribution $p$ into $p'$ as
\[
	p' = M p.
\]
Having the matrix $M$ and an initial state $p(0)$, the distribution after $m$ steps is described by the formula
\begin{equation}
	p(m)=M^m p(0).
	\label{eq:cevolution}
\end{equation}
The allowed transitions (steps) of the random walker from position $i$ to position $j$ are reflected within $M$ by the condition $M_{ji}\neq 0$. For now, we also assume (although it is not necessary) a weak form of symmetry in the transitions by requiring that $M_{ij}$ is also not zero. Forbidden transitions correspond to the condition $M_{ji}=M_{ij}=0$. The allowed transitions reflected in the non-zero elements of $M$ induce a graph structure $\mathcal G=(V,E)$ on $\Omega$. Here $V=\Omega$ is a set of vertices (corresponding to states) and $E=\{(j,i)\st j,i\in\Omega,M_{ji}\neq0\}$ is a set of ordered pairs of vertices (oriented edges, corresponding to transitions) -- the allowed connections between vertices. Conversely, we may say that the graph structure defines allowed transitions. For simplicity, from now on we will use the notation $ij$ instead of $(i,j)$ for the oriented edges.
%For symmetrical transitions, where $M_{ji}=M_{ij}=0$ it is enough to set $E=\{\{j,k\}\st j,k\in\Omega,M_{jk}\neq0\}$.

The graph structure is not the only thing reflected in $M$. The coefficients of $M$ also define the transitional probabilities to different states and in this manner reproduce the behaviour of the stochastic generator, usually called a \emph{coin}. For an \emph{unbiased coin,} which treats all directions equally, the coefficients of $M$ are defined as
\begin{equation}
\label{eq:unbiasedRW}
M_{ji}=\begin{cases}
\frac{1}{d(i)} & \text{for $(i,j)\in E$,}\\
0 & \text{otherwise,}\end{cases}
\end{equation}
with $d(i)$ being the degree of the vertex $i$. If this is not true, we say that the coin is \emph{biased}, preferring some directions above others.


%=============================================================================================
\subsection{Properties of Random Walks}
\label{sec:RWproperties}

When studying properties of random walks we search for specific properties that (potentially) help us solve various posed problems. Sometimes we want to know where the walker is after some time, in other cases we may want to know how much time does the walker take to arrive at some position or what is the probability of the walker to get there in given time. Another question asks how much time we need to give the walker so that finding him in any position has approximately the same probability. All these questions are not only interesting, but also useful for the construction (and understanding) of randomized algorithms.

If we are concerned with an unbiased random walk in one dimension (the so called drunkard's walk introduced in the previous Chapter), according to the central limit theorem, the distribution very quickly converges to a Gaussian one. The standard deviation of the position of the walker becomes proportional to $\sqrt{m}$, where $m$ is the number of steps taken. Such an evolution describes a diffusive process.
%A simple proof can be found e.g.~in Ref.~\cite{Kvasnica83}(?) and we present it in shortened form.

All the routes to get from position $0$ to position $x$ (positive or negative) after performing $m$ steps are composed of $n_+=(m+x)/2$ steps upward and $n_-=(m-x)/2$ steps downward. This is under supposition of what we shall call \emph{modularity} -- after an even (odd) number of steps, the probability to find the walker on odd (even) positions is always zero, constraining $m+x$ to be even (this is consequence of bipartite character of the graph). The number of these paths characterized by specific $n_\pm$ is
\[
N(x,m)={m\choose n_+}=\frac{m!}{n_+!n_-!}.
\]
The number of all possible paths is $N(m)=2^m$ and, hence, the probability to find the walker at position $x$ is $P_\mathrm{rw}(x,m)=N(x,m)/N(m)$. Using Stirling's approximation
\[
n!\sim\sqrt{2\pi n}\left(\frac{n}{\e}\right)^n,
\]
we can express the probability of finding the walker at $x$ after $m$ steps as
\begin{eqnarray*}
	P_\mathrm{rw}(x,m) &=& \frac{m!}{2^m\,n_+!n_-!}\\
	 & \simeq & \sqrt{\frac{2}{m\pi}}\left[\left(1+\frac{x}{m}\right)\left(1-\frac{x}{m}\right)\right]^{-\frac{m}{2}}
	 		\left(1+\frac{x}{m}\right)^{-\frac{x-1}{2}}\left(1-\frac{x}{m}\right)^{\frac{x-1}{2}} \\
	& \simeq & \sqrt{\frac{2}{m\pi}}\left[1-\frac{x^2}{m^2}\right]^{-\frac{m}{2}},
%\to \sqrt{\frac{2}{m\pi}}\e^{-\frac{x^2}{2m}}, x\ll m.
\end{eqnarray*}
where we assumed $m\gg x$, making the last two terms in the second line approximately one. In the limit of large $m$ and small $x$, this approximation can be  further transformed into the formula\footnote{Employ $\lim_{x\to\infty}\left(1-\frac{1}{x}\right)^x=\e$.}
\[
P_\mathrm{rw}(x,m)\simeq\frac{2}{\sqrt{2\pi m}}\exp\left(-\frac{x^2}{2m}\right).
\]
The function $P_\mathrm{rw}$ is not yet a probability distribution as it is normalized to $2$, but we have to recall the modularity of the walk telling us, that after even number of steps, the walker cannot be on odd position and after odd number of steps, the walker cannot be on even position; this leads us to a probability distribution having form
\begin{equation}
	\label{eq:pdf_rw}
	p_\mathrm{rw}(x,m)=\frac{1+(-1)^{m-x}}{\sqrt{2\pi m}}\exp\left(-\frac{x^2}{2m}\right).
\end{equation}
Finally, we observe
\begin{equation}
	\label{eq:rw_slimak}
	\langle x^2\rangle\equiv\sum_{x=-\infty}^\infty x^2 p_\mathrm{rw}(x,m)
	\simeq\frac{1}{2}\int_{-\infty}^\infty x^2 P_\mathrm{rw}(x,m) \dd x=m,
	\qquad
	\sqrt{\langle x^2\rangle}=\sqrt{m},
\end{equation}
where we approximated the modular probability distribution by a smooth one, $P_\mathrm{rw}/2$. 

The standard deviation of a walker is thus proportional to $\sqrt{m}$, and this fact may be deduced even without the knowledge of the limiting distribution (see e.g.~Ref.~\cite{Hughes}). The position of the walker $x$ is in fact a sum of $m$ independent variables (steps up and down) $y_1, \ldots, y_m$:
\[
x=\sum_{j=1}^m y_j.
\]
The square of the standard deviation then reads
\[
	\sigma^2(m) = \langle |x-\langle x\rangle|^2\rangle = \langle x^2\rangle-\langle x\rangle^2
	= \biggl\langle \sum_{j=1}^m y_j\sum_{l=1}^m y_l\biggr\rangle-\bigl\langle \sum_{j=1}^m y_j\bigr\rangle^2.
\]
As the $y_j$'s are independent, the sums and averages can be exchanged, giving us
\[
	\sigma^2(m)=\sum_{j=1}^m\sum_{l=1}^m\bigl(\langle y_jy_l\rangle-\langle y_j\rangle\langle y_l\rangle\bigr).
\]
For $j\neq l$, the independence of the random variables $y_j$ is reflected in $\langle y_jy_l\rangle=\langle y_j\rangle\langle y_l\rangle$, so the square of the standard deviation simplifies to
\[
	\sigma^2(m)=\sum_{j=1}^m\bigl(\langle y_j^2\rangle-\langle y_j\rangle^2\bigr)=\sum_{j=1}^m\sigma^2_j=m\sigma^2,
\]
where $\sigma_j$ are standard deviations of the random variables $y_j$. In this case, they are are all the same and equal to $\sigma_j\equiv\sigma=1$. Thus we finally arrive at $\sigma(m)=\sqrt{m}$ by a different route.

There are also other simple observations we can make. Let us list them here, with the aim of later comparing them to the properties of the distributions arising from quantum walks.

\paragraph{Reaching an absorbing boundary.}\label{sec:classicalabsorbingboundary}
Let us look at the probability with which the walker returns into its starting position. After leaving this position, the walker makes a move forward. Now there is probability $p_{10}$ for him to get back to the original position by taking all the possible routes into consideration. Under closer inspection, we find that this probability consists of the probability for him to make one step backward, which is $1/2$ and the probability for him to get back to the initial position only after moving further away from it first. This latter probability equals $\frac{1}{2}p_{10}^2$, since he moves forward with probability $1/2$ and then has to move two steps back with equal probabilities $p_{10}$ (we suppose, that no matter how far from the initial position the walker is, he always has equal probabilities to move forward and backward). To sum up, we see that
\[
p_{10}=\frac{1}{2}+\frac{1}{2}p_{10}^2.
\]
The only solution to this quadratic equation is $p_{10}=1$. Let us interpret this result: the probability for the walker to return to his initial position is equal to one, i.e.~he always gets back. 
In other words, if we employ an \emph{absorbing boundary} at position 0 and start at position 1, the walker will eventually hit the boundary.

This result can be extended to the statement that the probability of reaching vertex $i$ from any other vertex $j$ is one. As the walk is translationally symmetric, the probability to get from any $x$ to $x\pm 1$ at any time is always the same, $p_{10}=1$. Thus, the probability to get from $j$ to $i$ is
\begin{eqnarray}
	p_{ji}=p_{10}^{|j-i|}=1. \label{classicalabsorb}
\end{eqnarray}
This is quite different from quantum walks, where the probability to hit some boundary is not one, as shown in Sec.~\ref{sec:discreteboundary}.

\begin{exercise}
What is the probability $p_{10}$ in general case, when the probability to move right is $p$ and the probability to move left is $1-p$ in each step?
\end{exercise}

%\comment{Aj sem hodime uz nejaky predkrm o porovnani s quantum? Alebo tam absorbing boundary nerobime?}

\paragraph{Limiting distribution.}
Now\label{page:convergence} let us step away from the example of a walk on a linear chain and look at the larger picture, considering general graphs. For these, two quantities describing the properties of random walks are widely used in the literature --- the \emph{hitting time} and the \emph{mixing time}. But first, let us have a closer look at walks with unbiased coins on finite graphs. It is interesting to find, that all such graphs (if connected and non-bipartite) converge to its stationary distribution $\pi=(d(1),d(2),\ldots,d(N))/2|E|$, where $d(j)$ stands for the degree of vertex $j$. It is easy to see that this is a stationary distribution. For any vertex $j$ we have
\[
(M\pi)(j)=\sum_{i\st ji\in E}M_{ji}\pi(i)=\sum_{i\st ji\in E}\frac{1}{d(i)}\frac{d(i)}{2|E|}=\frac{d(j)}{2m}=\pi(j).
\]
This distribution is clearly uniform for regular graphs. In Appendix \ref{sec:classicallimit} we also provide a proof that for connected and non-bipartite graphs, this distribution is unique and also is the limiting distribution. With this notion we are ready to proceed to define the quantities of hitting and mixing time.

\paragraph{Hitting time.}
It is the average time (number of steps) that the walker needs to reach a given position $j$, when it starts from a particular vertex ($c$ stands for \emph{classical})
\begin{equation}
	\label{eq:classical_hitting}
	h^\mathrm{c}(j)=\sum_{m=0}^\infty m\, p(j,m).
\end{equation}
This quantity also makes sense for infinite graphs. We will later see (in Sec.~\ref{sec:discretehitting}) that for quantum walks this quantity is defined differently, due to the fact that measurement destroys the quantum characteristics of the walk.
%We will concentrate on properties of hitting times for random walks later, when we will be concerned with particular graph structures and their comparison with quantum ones.

\begin{example}
We have seen, that when the walker starts at position $1$ she will eventually reach position $0$. Let us evaluate now the hitting time between these two positions. As the number of paths of length $2k$ which do not get to position 0 is determined by catalan number $C_k$ (see Appendix \ref{sec:catalan_numbers}), the probability for the walker to hit vertex $0$ after $2k+1$ steps is
\[
p_{2k+1}\geq\frac{C_k}{2^{2k+1}},
\]
where the inequality sign comes from the fact that we counted all $2^{2k}$ paths, even those crossing and/or hitting 0. When we employ Eq.~(\ref{eq:classical_hitting}) and Eq.~(\ref{eq:catalan_bound}) we find, that
\[
h^\mathrm{c}(1\to 0)\geq\sum_{k=0}^\infty \frac{(2k+1)C_k}{2^{2k+1}} \geq \frac{\sqrt{\pi}}{\e^2}\sum_{k=0}^\infty\frac{1}{\sqrt{2k+1}},
\]
which diverges and so the hitting time is infinite.
\end{example}

\begin{exercise}
Consider now, that the probability to jump from position $1$ to $0$ is $p>0$. Starting at position $1$ we wait for one step and look whether the walker hit the boundary. If not we again set the walker to position $1$ and repeat procedure again and again until we hit the boundary. Show that in such experiment the hitting time is
\begin{equation}
\label{eq:hitting_analogue}
h^\mathrm{c}(1\to 0)=\frac{1}{p}.
\end{equation}
In this case the hitting time is finite. We could as well let the walker go for some time $T$ in which case the probability of hitting the boundary within this time would be some other $p$ but the hitting time would be expressed in the same way as in Eq.~(\ref{eq:hitting_analogue}). This definition leads to the emergence of tuples $(T,p)$ with the hitting time given by Eq.~(\ref{eq:classical_hitting}) being just a special case basically when $p<1$ for $T\to\infty$. Such definition seems to coincide more with the notion of absorbing boundary --- the probability of absorption is the smallest $p$ for which $(\infty,p)$ describes correct analouge of the hitting time given by Eq.~(\ref{eq:hitting_analogue}). See also definition of hitting time in the quantum case in Sec.~\ref{sec:discretehitting}.
\end{exercise}

\paragraph{Mixing time.}
The second important quantity is the classical \emph{mixing time} $\mathcal M_\epsilon^\mathrm{c}$. 
As we have seen each unbiased random walk (on connected non-bipartite graphs) reaches a stationary distribution, which we denote $\pi$.
The mixing time is then the time (number of steps) after which the probability distribution remains $\epsilon$-close to the stationary distribution $\pi$, i.e.
\begin{equation}
	\label{eq:classical mixing}
	\mathcal M_\epsilon^\mathrm{c}=\min\{T\st\forall t\geq T, \no{p(\cdot,t)-\pi(\cdot)}_{tvd}\leq\epsilon\},
\end{equation}
where $p(\cdot,t)$ is the distribution in time $t$ and $\no{\ \cdot\ }_{tvd}$ is (total variational) distance of distributions,
\begin{equation}
	\label{eq:TVD}
	\no{p(\cdot,t)-\pi(\cdot)}_{tvd}\equiv\sum_{j}\no{p(j,t)-\pi(j)}.
\end{equation}
Again, we will later see in Sec.~\ref{sec:discretemixing} that the mixing time is defined differently for quantum walks, as they are unitary and converge to a stationary distribution only in a time-averaged sense.

In classical case mixing time depends on the gap between the first two eigenvalues $\lambda_1=1$ (for the stationary distribution $\pi$) and $\lambda_2$. The use is illustrated by the next theorem.
\begin{theorem}[Spectral gap and mixing time]
\[
\frac{\lambda_2}{(1-\lambda_2)\log 2\epsilon}\leq \mathcal M_\epsilon^\mathrm{c}.
\]
\end{theorem}
For closer details see e.g.~Ref.~\cite{Sinclair93}.

\begin{example}[Traversing a hypercube]
\label{ex:traversing_hypercube}
An $n$-dimensional {\em hypercube} is a graph with vertices that are binary strings of length $n$ (see Fig.~\ref{fig:hypercubefigure}). For every pair of vertices $a$ and $b$ we can define \emph{Hamming distance,} which is the number of positions in which the two binary representations of $a$ and $b$ differ. Clearly this is the smallest number of steps one has to make in order to get from the vertex $a$ of the hypercube to the vertex $b$ as two vertices are connected by an edge if and only if the two strings corresponding to the vertices differ only by a single bit (thus have Hamming distance 1). In the hypercube, we can further distinguish a layered structure. Let us label two opposite vertices of the hypercube \textsc{entrance} and \textsc{exit}. We say, that vertex $a$ is in the layer $k$, if its Hamming distance from the \textsc{entrance} vertex is $k$. We can see, that any $k$-th level vertex has neighbours only in levels $k-1$ or $k+1$. Also note, that \textsc{entrance} vertex has Hamming distance $0$ and \textsc{exit} vertex has Hamming distance $n$.

Starting at the \textsc{entrance} vertex, our aim is to get to the \textsc{exit} as fast as possible. As between \textsc{entrance} and \textsc{exit} vertices there is rougly $2^n$ other vertices, usual random walk approach would find \textsc{exit} only in time exponential in $n$ --- the hitting time is $O(2^n)$ and as a result mixing time is even longer.

We can however radically shorten the time needed when we employ the walker with memory helping the walker to advance through the hypercube and increase her Hamming distance from the \textsc{entrance} in each step --- see algorithm in Fig.~\ref{fig:hypercube_alg}. Let us label vertices the walker visits as $a_k$, with index $k$ denoting the step (and layer as well). From the \textsc{entrance} vertex, denoted as $a_0$, the walker moves to random neighbour $a_1$, remembering the vertex it came from in memory $S_0=\{a_0\}$. The memory will contain all the vertices that are from lower layer, than actual vertex. Clearly, for $S_0$ this is true.

On each step $k+1$ the walker chooses new neighbour $a_{k+1}$ of actual vertex $a_k$ from the next $(k+1)$-th layer by excluding the vertices from memory $S_{k-1}$ from the selection process, as these are from layer $k-1$. New memory $S_k$ is constructed as a set of all neighbouring vertices of $a_{k+1}$ that are also neighbours of some of the vertices in $S_{k-1}$.

To see that it works as intended, let us say, that $a_{k+1}$ was obtained from $a_k$ by flipping bit at position $q$. From definition of $S_{k-1}$ we know, that $a_k\not\in S_{k-1}$ and so all vertices contained in this set differ from $a_{k+1}$ in two bits, $q$ and some $r\neq q$. Now, to get from $a_{k+1}$ to lower level, we would have to go either to $a_k$, which is a neighbour of $S_{k-1}$, or we would flip the bit on position $r$ taking it to one-bit-flip ($q$) from some vertex from $S_{k-1}$.

\begin{figure}
\begin{algorithm}
Set $k=1$, the initial position $a_1$ to a random neighbor of the \textsc{entrance} vertex and $S_0=\{a_0\}$ then for $n-1$ times repeat:
\begin{enumerate}
\item set $k:=k+1$
\item randomly choose $a_k$ to be neighbor of $a_{k-1}$ such that $a_k\not\in S_{k-2}$
\item set $S_{k-1}$ to be the set of all neighbors of $a_k$ that have a neighbor also in $S_{k-2}$
\end{enumerate}
The resulting vertex is \textsc{exit}.
\end{algorithm}
\caption{\label{fig:hypercube_alg} Algorithm for traversing the $n$-hypercube. Starting at position \textsc{entrance} the walker uses structural oracle to navigate through the graph. She has to remember only $O(n)$ vertices in each step which help her propagate thorugh the graph increasing the layer in each step.}
\end{figure}

It is easy to see now, that $S_k$, as a memory, is a set of all neighbours of vertex $a_{k+1}$ that are at level $k$. In this manner the walker in each step increases its distance from the \textsc{entrance} vertex and decreases its distance from the \textsc{exit} vertex, thus needing $n$ steps to traverse the graph with $\order(n)$ searches in neighbourhood every step. Totally the efficiency of the algorithm is polynomial in $n$ with memory of $O(n)$.
\end{example}


==> komentareNagaj.tex <==
%---------------------------------------------------------------------------------------
%--- este nevyriesene
%---------------------------------------------------------------------------------------


Section 3.4 

Tu som na konci dal poznamku o inych typoch oraclov. Ten treti je to, co sa v grafovych ulohach naozaj pouziva... A potom Sekcia 3.5 s prikladom hviezdicky potrebuje O(N^2) klasicky, O(N) kvantovo, a dava lower bound na triangle problem. Ty pouzivas 2.typ, ktory HNED vypluje zoznam susedov. Mam pocit, ze 3ti je prirodzenejsi.


koniec 3ky, pridat [citacie]


DN opravi este 1.3 subor.

%---------------------------------------------------------------------------------------
%--- zoznam vsetkych
%---------------------------------------------------------------------------------------
Kapitola 1

3 - ideal paramagnetic gas - footnote, viac vysvetlit
3 - kinetic theory - footnote, jednou vetou vysvetlit
4 - barometric formula - co to je a naco to je? footnote?
4 - stochastic moves - chce to footnote? co to znamena? iba dat do zatvorky (random)?
6 - veta o "modularity" ... nerozumiem
8 - absorbing boundary: 
	-	Da sa dokazat aj to, ze ked zacneme nielen 1 od boundary 
		ale kdekolvek, chytime ho? Dajme to tam!
	-	Aj sem hodime uz nejaky predkrm o porovnani s quantum? 
		Alebo tam absorbing boundary nerobime?
   - pridat odkaz na to, kde v q.walks su definovane hitting times
   - co znamena veta o zmysluplnosti pre nekonecne grafy?
   - co znamena horny index c? zaciatocny bod? 
   - to iste v Mixing time
   - v Mixing time zaviest stationary distribution... dokazat to! (dat napriklad do appendixu, je to celkom pekna vec, spravit jasne podmienky) dat citaciu
   
Kapitola 2

22 - under the given approximations (ake su to?)
22 - shows that the dispersion grows (je to disperzia? odmocnina? nevadi to, ze stredna hodnota x je nenulova? mozno by som to tam dopisal)
23 - prepisal som trochu Exercise 5. Je to teraz to, co si chcel?

Po minciach, koniec 2.4 pridat Grovera, vypocet pravdepodobnosti (aj "Hitting time") s tou mincou, co sme prave nasli. 
V spojitom case ma DanoN oddelenie 5.2.
Pozriet aj Ambainisa.

27. combined action of the local... je to U = \bigotimes_{k=1}^{N} U^{(k)}?
TO predsa nie je take jednoduche, ci? Ako to citatelovi lepsie vysvetlit?
Lebo ides z Omega_k do A_k, co ma prekryv so vsemoznymi inymi Omega_m...

este pekny obrazok k tomu, aby to ludia pochopili hned? nemas nieco v phd.praci?

-----------

28. obrazok Fig.6 - mas tam nesymetricku dot-dashed, velmi slabo je ju vidno... co tak hrubsiu ciaru?

sekcia 2.4.1 som riadne prehadzal. Precitaj si to, prosim.
Dal som footnote o unbiased coins being equivalent. Je to pravda?

Sekcia 2.4.2
strana 29
Co znamena, ze sa nemeni degree of spreading, ale meni sa extent? Tu vetu som vobec nepochopil. 

36 - nejake otazky v texte o mixing time

2.5.2 strana 37
Footnote: FeHi definovali jednu vec ci dve? Zhodnu sa oni sami medzi sebou, alebo s Kempe 05?

2.5.3 strana 38
O com je ten exercise? Ze nikdy neskocis z 1 do -1? Ale z 0 uz do -1 pojdes, nie? Nerozumiem.

Figure 13: co su tie male horizontalne ciary???

-----------

Section 3

strana 41 - co je znamena poznamka o "different coin" v algoritme pre hypercube search?

o com je to o two-dimensional reduction? nerozumiem VOBEC.

43 - the oracle may well be a subroutine
tej vete nerozumiem

----------

Section 3.2

o co ide v tom ze dimensionality of the problem is beyond the theory given in 33? Nechapem. Dimenzia vertexov? Dimenzia celeho priestoru? Je to matuce. Obe tieto chapania su predsa mensie... alebo preto, ze analyza potrebuje viac dimenzii?


Section 3.4

Tu som na konci dal poznamku o inych typoch oraclov. Ten treti je to, co sa v grafovych ulohach naozaj pouziva... A potom Sekcia 3.5 s prikladom hviezdicky potrebuje O(N^2) klasicky, O(N) kvantovo, a dava lower bound na triangle problem. Ty pouzivas 2.typ, ktory HNED vypluje zoznam susedov. Mam pocit, ze 3ti je prirodzenejsi.

strana 60.
Preco je tak vybraty zaciatocny stav? Nepochopil som to vysvetlenie.

strana 62. 
Vselico som pripisal, ale mam tam podstatnu otazku (je v texte).

strana 64.
dve otazky - average/worst case, a walk on a complete graph (su v texte ako comment)



==> odpad.tex <==
% ------------------------------------------------------------
% ------------------------------------------------------------
% ------------------------------------------------------------
% ------------------------------------------------------------
% ------------------------------------------------------------

JORDAN'S LEMMA

Consider now an $N$-dimensional Hilbert space $\cH$, a rank $r$ projector
$\Pi_1$ and a rank $s$ projector $\Pi_0$, with $1\le r, s \le N$. 
Jordan's lemma implies the existence of an orthonormal basis for the Hilbert space
$\cH$ which can be divided into five groups. 
\begin{enumerate}
\item Two-dimensional
		subspaces $S_i$ for $i=1,\dots,t$, invariant under both $\Pi_1$ and $\Pi_0$. Each
		subspace $S_i$ is spanned by the orthonormal eigenvectors $\ket{v_i}$ and $\kets{v_i^{\perp}}$
		of the projector $\Pi_1$, i.e. obeying 
		$\Pi_1 \ket{v_i} = \ket{v_i}$ and  $\Pi_1\kets{v_i^{\perp}} = 0$.
\item Four types of one dimensional subspaces $T^{(bc)}_i$, where $b,c\in\{0,1\}$. These 
		$N-2t$ subspaces are spanned by $\kets{v^{(bc)}_i}$, for $b,c\in\{0,1\}$,
		obeying
		\begin{eqnarray}
			\Pi_1 \kets{v^{(bc)}_i} = b \kets{v^{(bc)}_i}, \qquad
			\Pi_0 \kets{v^{(bc)}_i} = c \kets{v^{(bc)}_i}. 
			\label{onedim}
		\end{eqnarray}
\end{enumerate}

The 2D subspaces $S_i$ can be also spanned by the orthonormal
eigenvectors $|w_i\rangle, |w_i^\perp\rangle$ of the projector $\Pi_0$,
satisfying $\Pi_0 |w_i\rangle =|w_i\rangle$ and $\Pi_0 \kets{w_i^\perp} =0.$
Hence, we can recast the projectors $\Pi_1$ and $\Pi_0$ in the form 
\begin{eqnarray}
\label{basis_h}
 \Pi_1 &=& \sum_{i=1}^{t} \ket{v_i}\bra{v_i} 
 			+ \sum_{i} \kets{v^{(10)}_i}\bras{v^{(10)}_i} 
 			+ \sum_{i} \kets{v^{(11)}_i}\bras{v^{(11)}_i}, \\
 \Pi_0 &=& \sum_{i=1}^{t} \ket{w_i}\bra{w_i} 
 			+ \sum_{i} \kets{v^{(01)}_i}\bras{v^{(01)}_i} 
 			+ \sum_{i} \kets{v^{(11)}_i}\bras{v^{(11)}_i}.\nonumber
\end{eqnarray} 
in terms of our chosen orthonormal basis of the Hilbert space $\cH$.


--------

Proof of the spectral theorem

\begin{proof}
With a suitable choice of the orthonormal eigenvectors
$\{|w_i\rangle, |w_i^\perp\rangle \}$ of the projector $\Pi_0$ 
and defining\footnote{Note that in \eqref{principal}, we chose to use
the rescaled $\varphi_i=\frac{\theta_i}{\pi}$ instead, to unify the notation with phase estimation.}
 the principal angle $\theta_i$
\begin{eqnarray}
		\cos\theta_i=|\langle v_i | w_i \rangle|,
\end{eqnarray}
we can write the transformation law
\begin{eqnarray}
	\kets{v_i} &=& \phantom{-} \cos \theta_i \kets{w_i} + \sin \theta_i \kets{w_i^\perp}, \\
	\kets{v_i^\perp} &=& - \sin \theta_i \kets{w_i} + \cos \theta_i \kets{w_i^\perp}.
\end{eqnarray}
between the two bases as
\begin{eqnarray}
	\left(\begin{array}{l}
			\kets{w_i}\\
			\kets{w_i^\perp}
		\end{array}\right)
	= U   
		\left(\begin{array}{l}
 			\kets{v_i} \\
 			\kets{v_i^\perp}
		\end{array}\right),
\end{eqnarray}
where the transformation
\begin{eqnarray}
	U = e^{i \theta_i \hat{\sigma}_y} = \ii \cos \theta_i + i \hat{\sigma}_y \sin\theta_i
\end{eqnarray}
is a unitary rotation. 
Therefore, $(2\Pi_1-\ii)(2\Pi_0-\ii)$ expressed in the basis $\{\kets{v_i},\kets{v_i^\perp}\}$ is
\begin{eqnarray}
	(2\Pi_1-\ii)(2\Pi_0-\ii) 
	&=&
		\left[\begin{array}{rr}
				1 & 0\\ 
				0 & -1
		\end{array}\right]
		\underbrace{U
		\left[\begin{array}{rr}
				1 & 0\\ 
				0 & -1
		\end{array}\right]
		U^{\dagger}}_{2\Pi_0-\ii} \\
	&=& \hat{\sigma}_z e^{i \theta_i \hat{\sigma}_y} \hat{\sigma}_z e^{-i \theta_i \hat{\sigma}_y} 
	= \hat{\sigma}_z \hat{\sigma}_z e^{-i \theta_i \hat{\sigma}_y} e^{-i \theta_i \hat{\sigma}_y} \\
	&=& e^{-i (2\theta_i) \hat{\sigma}_y},  \label{PPform}
\end{eqnarray}
where we used the anticommutation relationship $\hat{\sigma}_z \hat{\sigma}_y + \hat{\sigma}_y \hat{\sigma}_z = 0$.
In each two-dimensional subspace $S_i$, the operator $(2\Pi_1-\ii)(2\Pi_0-\ii)$ is thus a rotation 
by $2\theta_i$. Moreover, its form is \eqref{PPform} also in the basis
$\{\kets{w_i},\kets{w_i^\perp}\}$, because $U^\dagger e^{-i (2\theta_i) \hat{\sigma}_y} U
=e^{-i (2\theta_i) \hat{\sigma}_y}$.

To conclude the proof, let us look at the action of $(2\Pi_1-\ii)(2\Pi_0-\ii)$ 
on the one-dimensional invariant subspaces.
Using \eqref{onedim}, we find that it acts as an identity on the subspaces $T^{(00)}_i$ and $T^{(11)}_i$
and as $-\ii$ on the subspaces $T^{(01)}_i$ and $T^{(10)}_i$.
\end{proof}





% ------------------------------------------------------------
% ------------------------------------------------------------
% ------------------------------------------------------------
% ------------------------------------------------------------
% ------------------------------------------------------------

SZEGEDY'S WALKS

\subsection{Bipartite walks}
Walking with two registers.
Doing the reflections.

Hard to quantize Markov chains that are not regular -- problems with
making the coin. That's why Szegedy took a different approach.
Using the state of the walk to actually ``make'' a coin.

[AN IMAGE OF A BIPARTITE WALK, $p_{x,y}$ arrows and such.]

Let us start with a classical bipartite walk on two sets $X$ and $Y$.
We can get a bipartite walk from any walk by simply doubling the state space. 
The transition matrix then looks like
\be
	M = \left[ \begin{array}{cc}
				0 & Q\\
				P & 0
	\end{array} \right]
\ee
with $P=(p_{x,y})$ containing the transition probabilities from going from $X \goes Y$ and $Q=(q_{y,x})$ the matrix of transition probabilities for the map 
$Y \goes X$. We have $\sum_{y}p_{x,y}=1$ and $\sum_{x}q_{y,x}=1$.

Make it all much simpler by taking $p_{x_y}=q_{y,x}$ and consider the doubling
of a regular walk -- or simply symmetric bipartite walks.
Now go back to having $p_{x,y}=q_{y,x}$, i.e. the matrices $P=Q$ and thinking of making a simple walk into a bipartite by doubling\dots

How do we quantize such a walk? We will consider a quantum system with two registers
$\cH_{left}\otimes \cH_{right}$. 
We need to come up with a unitary operation that would mix things up on the two registers. 
The pure state with two registers
\be
	\ket{\phi_x} &=& \ket{x} \otimes \left(\sum_{y\in X} \sqrt{p_{x,y}} \ket{y}\right). \label{bipartphi}
\ee
is encoding what we would get by one step of the original walk
when starting in the state $x$.
We choose our mixing unitary to be a reflection about the subspace spanned by all the states $\ket{\phi_x}$, i.e.
\be
	R_1 = 2 \left(\sum_{x\in X} \ket{\phi_x}\bra{\phi_x}\right) - \ii.
\ee
Similarly, with the help of the states 
\be
	\ket{\psi_y} &=& \left(\sum_{x\in X} \sqrt{p_{x,y}}\ket{x}\right) \otimes \ket{y} \label{bipartpsi}
\ee
with the registers swapped compared to \eqref{bipartphi}, we define a second reflection 
\be
	R_2 = 2 \left(\sum_{y\in Y} \ket{\psi_y}\bra{\psi_y}\right) - \ii.
\ee
Together, these two reflections make up one step of the quantized version of the bipartite walk as
\be
	W = R_2 R_1.
\ee


The state invariant under both of these reflections is
\be
	\ket{\psi} = \sum_{x\in X}\ket{\varphi_x} = \sum_{y\in Y}\ket{\psi_y}
	= \sum_{x\in X}\sum_{y \in Y} \sqrt{p_{x,y}} \ket{x}\ket{y}.
\ee

%=============================================================================================
%\subsection{Vedierko}

%In fact, Brownian motion can be described by a physically interpretable Langevin equation
%\[
%m\frac{\dd\mathbf v}{\dd t}=\mathbf F(\mathbf r)-\beta\mathbf v+\pmb\eta(t).
%\]
%This is an equation of the motion for a particle with mass $m$ in potential described by interactions via $\mathbf F(\mathbf r)$ and under the influence of the viscous force (with coefficient $\beta$) and time dependent noise described by the last term $\pmb\eta(t)$. This formula describes a physics of random movement of the system and is a usual choice in many subfields of physics.

%After this introduction to random walks, we can now compare the structure of quantum\footnote{This comparison holds for discrete-time quantum walks that will be introduced in Sec.~\ref{sec:DTQW}. For continuous-time random walks the relationship with their classical counterparts --- continuous Markovian processes --- is clear from construction (see Sec.~\ref{sec:CTQW}).} and random walks. While in random walks the state of the walker (its distribution) is defined by a tuple of real numbers representing probabilities, in quantum walks the state is defined by a unit vector from corresponding Hilbert space. The graph structure in classical case is reflected in the non-zero elements of stochastic matrix $M$ and in quantum case is defined by the translational operator $\op S$ having the same meaning as the adjacency matrix in classical case, that defines the connections in graph by having elements of value one for connected vertices and zero otherwise. The coin in classical case is reflected in the size of the coefficients of $M$ but in quantum case, for reasons explained in Sec.~\ref{sec:coins}, we have to employ another degree of freedom for the coin and unitary matrix $\op C$ acting on this degree of freedom. Finally, the evolution is described very similarly in both cases --- in classical by Eq.~(\ref{eq:cevolution}) and in quantum as $\ke{\psi_m}=\op U^m\ke\psinit$ [see Eq.~(\ref{eq:qevolution})], where quantum evolution operator $\op U$ is composed of actions of $\op S$ and $\op C$. Seeing this connection between quantum and random walks we will later give further insight into what do they have in common and in what they differ.

%Finally, let us note, that the concept of random walk is very similar to the concept of Monte Carlo method. In many respects they may be considered equivalent. The difference is mainly conceptual and may be described as in Ref.~\cite{Kendon06} saying that the mathematical concept of random walks underpins such methods in computational physics as Monte Carlo method. This holds also for topics of dynamical maps or cellular automata which can be in some cases represented in the form of random walks.

